Fractional Fourier Domain PAPR Reduction

High peak-to-average power ratio (PAPR) has long posed a challenge for multi-carrier systems, impacting amplifier efficiency and overall system performance. This paper introduces dynamic angle fractional Fourier division multiplexing (DA-FrFDM), an innovative multi-carrier system that effectively reduces PAPR for both QAM and Gaussian signals with minimal signaling overhead. DA-FrFDM leverages the fractional Fourier domain to balance PAPR characteristics between the time and frequency domains, achieving significant PAPR reduction while preserving signal quality. Furthermore, DA-FrFDM refines signal processing and enables one-tap equalization in the fractional Fourier domain through the simple multiplication of time-domain signals by a quadratic phase sequence. Our results show that DA-FrFDM not only outperforms existing PAPR reduction techniques but also retains efficient inter-carrier interference (ICI) mitigation capabilities in doubly dispersive channels.

==> ICI_derivation.tex <==
In addition to PAPR reduction, our DA-FrFDM has an inherent advantage over traditional OFDM systems in that it effectively mitigates the intercarrier interference (ICI) in doubly dispersive channels, i.e., frequency-selective fast fading channel, as the frequency of a specific subcarrier in DA-FrFDM varies over time at a rate of $\cot{\alpha}$.

Consider a doubly dispersive channel, after passing the channel, the signal received at the receiver can be written as
\begin{equation}
r(t)=\sum_{i=1}^Ph_i \widetilde{x}(t-\tau_i)e^{-j2\pi f_it}+n(t),
\end{equation}
where $P$ is the number of paths; $h_i$, $\tau_i$, and $f_i$ denote the gain, delay, and Doppler shift of each path. 

In such a doubly dispersive channel, ICI is inevitable, and the system becomes an interference-limited system. Therefore, we simply ignore the noise term in the following analysis. After processing at the receiver, the signal after DFrFT can be written as
\begin{equation}\label{eq:ydispersive}
\begin{aligned}
Y[m]&=\int\limits_{0}^{T}y(t)\sqrt{\frac{|\sin\alpha| - j\text{sgn}(\sin\alpha)\cos\alpha}{N}}\\
&\times e^{\frac{j}{2}t^2\cot\alpha} e^{\frac{j}{2}m^2\cot\alpha(\Delta u)^2} e^{-j2\pi mt/T}dt\\
&=\frac{1}{N} \sum_{k=0}^{N-1} X[k] e^{\frac{j}{2} (m^2 - k^2) \cot \alpha (\Delta u)^2}\\
&\times \sum_{i=1}^{L} e^{- \left(\frac{j 2 \pi k \tau_i}{T} + \frac{j}{2} \tau_i^2 \cot \alpha \right)}\\
&\times \int_0^T h_i(t) e^{j \frac{2 \pi (k - m) t}{T} + j t \tau_i \cot \alpha - j 2 \pi f_i t}  dt.
\end{aligned}
\end{equation}

According to \cite{2019.0962,7165663}, the ICI power is (considering power normalization)
\begin{equation}\label{eq:P_ICI}
\mathbb{E}_m[\sum_{k=0,k\neq m}^{N-1}|c_{m,k}|^2],
\end{equation}
 where
\begin{align*}
    c_{m,k} &= \frac{1}{T} e^{\frac{j}{2} (m^2 - k^2) \cot \alpha (\Delta u)^2} \sum_{i=1}^{L} 
     e^{- \left(\frac{j 2 \pi k \tau_i}{T} + \frac{j}{2} \tau_i^2 \cot \alpha \right)} \\
    & \times \int_0^T h_i(t) e^{j \frac{2 \pi (k - m) t}{T} + j t \tau_i \cot \alpha - j 2 \pi f_i t} \, dt.
\end{align*}

==> SecV_save.tex <==


% CCDF
% N=16 (gaussian), N=32 (gaussian), N=64 (gaussian, 64QAM)

% MSE
% N=16 (gaussian), N=32 (gaussian), N=64 (gaussian)

This section evaluates the PAPR performance of our DA-FrFDM scheme. We choose three PAPR reduction schemes for OFDM systems as benchmarks: clipping, SLM, PTS.

In the simulation, the number of subcarriers $N = 16$, $32$ or $64$, oversampling rate $L = 20$, and the symbol duration $T = 128~\mu s$. The data signals $\bm{s}$ follow a complex Gaussian distribution or are 64QAM signals, respectively.
\hl{To discuss:} we set the total number of symbols be 1000 and $\Delta{\alpha_1} = \frac{1}{2000} \sin^{-1}\left(\frac{T^2}{\pi}\right)$. Since $\Delta{\alpha_1}$ is small enough, we just set $\Delta{\alpha_2}=\Delta{\alpha_1}$.


We choose the Complementary Cumulative Distribution Function (CCDF) as the PAPR performance indicator, which calculates the probability that the PAPR exceeds a certain threshold, providing a clear measure of how often high peaks occur. The CCDF of PAPR is
\begin{equation}\label{eq:ccdf}
\text{CCDF}(\Gamma) =  \text{Pr}(\eta > \Gamma).
\end{equation}


\begin{figure}[t]
  \centering
  \includegraphics[width=0.87\columnwidth]{./g1016.pdf}\\
  \caption{CCDF of complex gaussian signals with different subcarrier numbers.\hl{run again}}
\label{fig.5}
\end{figure}

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=0.87\columnwidth]{./16QAM1002.png}\\
%  \caption{CCDF of 16QAM signals with different subcarrier numbers.}
%\label{fig.6}
%\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.87\columnwidth]{./64q1016.pdf}\\
  \caption{CCDF of 64QAM signals with different subcarrier numbers.\hl{run again}}
\label{fig.7}
\end{figure}





\subsection{PAPR comparison with other methods}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.87\columnwidth]{./spc_g1027.pdf}\\
  \caption{CCDF of complex gaussian signals of different PAPR reduction methods.}
\label{fig.papr_spc_g}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.87\columnwidth]{./spc_q1027.pdf}\\
  \caption{CCDF of 64QAM signals of different PAPR reduction methods.}
\label{fig.papr_spc_64q}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{./mse1027.pdf}\\
  \caption{MSE of complex gaussian signals based on different PAPR reduction methods.}
\label{fig.mse}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\columnwidth]{./ber1027.pdf}\\
  \caption{BER of 64QAM signals based on different PAPR reduction methods.}
\label{fig.ber}
\end{figure}




We set $N=64$ with a total of 1000 symbols. We compare DA-FrFDM with three conventional PAPR reduction methods: SLM, PTS, and clipping. The CCDF curves are shown in Figures~\ref{fig.papr_spc_g} and \ref{fig.papr_spc_64q}.

For the BER and MSE analysis, we set the total number of symbols to 3 and the number of iterations to 2000. The channel model is a traditional 6-path Rayleigh fading channel with AWGN. The BER and MSE performance for both complex Gaussian and 64QAM signals are illustrated in Figures \ref{fig.mse} and \ref{fig.ber}.

Similar to SLM, the core mechanism for reducing PAPR in our system involves multiplying the signal by a phase sequence. While classical SLM employs a phase sequence $\{\pm 1\}$, the DA-FrFDM system utilizes the phase sequence $e^{-\frac{j}{2}k^2\cot\alpha(\Delta u)^2}$.

In the PTS technique, the input data block is divided into $V$ disjoint subblocks:
\begin{equation}
\bm{x}=\mathrm{IFFT}\left\{\sum_{\nu=1}^{V}b^{\nu}\bm{s}^{\nu}\right\}=\sum_{\nu=1}^{V}b^{\nu}\cdot\mathrm{IFFT}\{\bm{s}^{\nu}\}=\sum_{\nu=1}^{V}b^{\nu}\bm{x}^{\nu}
\end{equation}
where $b^{\nu}$ are phase factors, traditionally chosen from $\{\pm 1\}$.

Clipping, on the other hand, limits the peak amplitude of the transmitted signal to a predefined threshold. Specifically,

\begin{equation}
x[n]=
\begin{cases}x[n]&\mathrm{if~}|x[n]|<A\\\\\frac{x[n]}{|x[n]|}\cdot A&\mathrm{otherwise},
\end{cases}
\end{equation}
where $A = \text{CR} \cdot \sigma$, with $\text{CR}$ being the clipping ratio and $\sigma$ the standard deviation of $x[n]$.


The number of phase sequence combinations/maximum operations in the SLM system is set to 128, and the number of subblocks in the PTS system is 8 (as given by $M = 2^{V-1}$). Additionally, we assume $\text{CR} = 2$ for the clipping method.


To maintain the same number of maximum operations, we set $\Delta{\alpha_1} = \frac{1}{80} \sin^{-1}\left(\frac{T^2}{\pi}\right)$ initially in the DA-FrFDM system, followed by $\Delta{\alpha_2} = \frac{\Delta{\alpha_1}}{39}$. Here, the number of maximum operations corresponds to the size of $\Omega_2$. Occasionally, when $\Omega_2 = \emptyset$ for some transmitted blocks, we set DFrFT to IFFT, which results in a single maximum operation. Through simulations, we find that the mean number of maximum operations per block of source symbols is 126.48 for complex Gaussian symbols and 126.868 for 64QAM symbols, both closely approximating 128.





The results show that the PAPR reduction performance of SLM, PTS, and clipping is inferior to that of DA-FrFDM. 

In terms of BER, DA-FrFDM, SLM, and PTS exhibit similar performance, while clipping results in worse BER performance.


\subsection{DA-FrFDM for eigenvalue decomposition based DFrFT}

Since eigenvalue decomposition-based DFrFT is not suitable for oversampling and does not align with Theorem~\ref{thm:1}, we set $L=1$, $\alpha \in [ 0, 2 \pi)$, and $\Delta \alpha = \pi \cdot 10^{-3}$. Figures~\ref{fig.ed} and \ref{fig.ed2} present the CCDF of PAPR in comparison with traditional OFDM, showing results that are on par with those achieved using sampling-based DFrFT.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.87\columnwidth]{./ed1016.pdf}\\
  \caption{CCDF of complex Gaussian signals with different subcarrier numbers (eigenvalue decomposition based DA-FrFDM). \hl{run again}}
\label{fig.ed}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.88\columnwidth]{./ed21016.pdf}\\
  \caption{CCDF of 64QAM signals with different subcarrier numbers (eigenvalue decomposition based DA-FrFDM).\hl{run again}}
\label{fig.ed2}
\end{figure}









%\begin{aligned}
%P_{\mathrm{ICI}}
%$&= \mathbb{E}_m \left[ \sum_{l=m-N+1}^{m} \sum_{i=1}^{L} \sigma_{i}^{2} \int_{-1}^{1} r(Tv)\left(1-|v|\right) \right. \\
%$& \left. \times e^{j(\tau_{i}\cot\alpha-2\pi f_{i})Tv} e^{-j2\pi lv} dv \right]
%\end{aligned}

% \noindent where $r(Tv)=J_0(2\pi f_dTv)$, $J_0$ is the zeroth-order Bessel function of the first kind.  





















% \subsection{ICI versus PAPR Tradeoff for DA-FrFDM in the XXX channels}
% In OFDM systems, subcarrier orthogonality eliminates intercarrier interference (ICI). Nonetheless, when operating in doubly dispersive channels, OFDM systems suffer from significant performance degradation due to the introduction of ICI. A major advantage of the FrFT-OFDM system is its ability to adapt to doubly dispersive channels, as the frequency of a specific subcarrier varies over time at a rate of $\cot{\alpha}$.


% After passing through a frequency-selective fast fading channel, the received signal becomes:


% \begin{equation}
% r(t)=\sum_{i=1}^Ph_i \widetilde{x}(t-\tau_i)e^{-j2\pi f_it}+n(t),
% \end{equation}
% where $P$ is the number of paths; $h_i$, $\tau_i$, and $f_i$ denote the gain, delay, and Doppler shift of each path; $n(t)$ is AWGN. 

% After removing the CP and taking DFrFT with angle $\alpha$,  the signal can be expressed as (assuming $n(t) = 0$):

% \begin{equation}\label{eq:Y[m]}
% \begin{aligned}
% Y[m]&=\int\limits_{0}^{T}y(t)\sqrt{\frac{|\sin\alpha| - j\text{sgn}(\sin\alpha)\cos\alpha}{N}}\\
% &\times e^{\frac{j}{2}t^2\cot\alpha} e^{\frac{j}{2}m^2\cot\alpha(\Delta u)^2} e^{-j2\pi mt/T}dt\\
% &=\frac{1}{N} \sum_{k=0}^{N-1} X[k] e^{\frac{j}{2} (m^2 - k^2) \cot \alpha (\Delta u)^2}\\
% &\times \sum_{i=1}^{L} e^{- \left(\frac{j 2 \pi k \tau_i}{T} + \frac{j}{2} \tau_i^2 \cot \alpha \right)}\\
% &\times \int_0^T h_i(t) e^{j \frac{2 \pi (k - m) t}{T} + j t \tau_i \cot \alpha - j 2 \pi f_i t}  dt.
% \end{aligned}
% \end{equation}

% According to \cite{2019.0962,7165663}, the ICI power is (considering power normalization)
% \begin{equation}\label{eq:P_ICI}
% \mathbb{E}_m[\sum_{k=0,k\neq m}^{N-1}|c_{m,k}|^2],
% \end{equation}

% \noindent where
% \begin{align*}
%     c_{m,k} &= \frac{1}{T} e^{\frac{j}{2} (m^2 - k^2) \cot \alpha (\Delta u)^2} \sum_{i=1}^{L} 
%      e^{- \left(\frac{j 2 \pi k \tau_i}{T} + \frac{j}{2} \tau_i^2 \cot \alpha \right)} \\
%     & \times \int_0^T h_i(t) e^{j \frac{2 \pi (k - m) t}{T} + j t \tau_i \cot \alpha - j 2 \pi f_i t} \, dt.
% \end{align*}









% Assume there are three paths with path gains of 0, -4.3429, and -8.6859 dB, and path delays of 0, 9, and 16 $\mu s$, respectively. Since $\alpha$ for the lowest ICI has already been derived in \cite{7165663}, we can simulate the $P_{ICI}$ versus PAPR curve under conditions of reduced $P_{ICI}$. It is important to note that we only simulate a smaller range of $\alpha$ than that specified in Theorem \ref{thm:1}. Although this range does not cover all possible PAPR values, it allows for a trade-off between PAPR and $P_{ICI}$, as illustrated in Figure~\ref{fig.ici}. The units of PAPR and $P_{ICI}$ are linear, not in dB. Therefore, we can draw straight lines between the local minimum points to determine the bound. This bound helps in selecting an appropriate $\alpha$.

% \begin{figure}[t]
%     \centering
%     \subfigure
%     [$a$ versus $\text{PAPR}$.]
%     {
%         \includegraphics[width=0.8\columnwidth]{./ici1016a.pdf}
%         \label{fig:sub1}
%     }
%     \subfigure
%     [$\cot\alpha$ versus $P_{ICI}$.]
%     {
%         \includegraphics[width=0.8\columnwidth]{./ici1016b.pdf}
%         \label{fig:sub2}
%     }
%     \subfigure
%     [$P_{ICI}$ versus $\text{PAPR}$.]
%     {
%         \includegraphics[width=0.8\columnwidth]{./ici1016c.pdf}
%         \label{fig:sub3}
%     }
%     \caption{Trade-off between PAPR and $P_{ICI}$.\hl{run again}}
%     \label{fig.ici}
% \end{figure}




